Towards Rehearsal-Free Multilingual ASR: A LoRA-based Case Study on Whisper

Pre-trained multilingual speech foundation models, like Whisper, have shown impressive performance across different languages. However, adapting these models to new or specific languages is computationally extensive and faces catastrophic forgetting problems. Addressing these issues, our study investigates strategies to enhance the model on new languages in the absence of original training data, while also preserving the established performance on the original languages. Specifically, we first compare various LoRA-based methods to find out their vulnerability to forgetting. To mitigate this issue, we propose to leverage the LoRA parameters from the original model for approximate orthogonal gradient descent on the new samples. Additionally, we also introduce a learnable rank coefficient to allocate trainable parameters for more efficient training. Our experiments with a Chinese Whisper model (for Uyghur and Tibetan) yield better results with a more compact parameter set.

==> _------- <==
%% Created for Prasanta Ghosh on -01-20

@inproceedings{vander2023using,
  title={Using adapters to overcome catastrophic forgetting in end-to-end automatic speech recognition},
  author={Vander Eeckt, Steven and Van Hamme, Hugo},
  booktitle={ICASSP 2023-2023 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={1--5},
  year={2023},
  organization={IEEE}
}
@article{yang2022online,
  title={Online continual learning of end-to-end speech recognition models},
  author={Yang, Muqiao and Lane, Ian and Watanabe, Shinji},
  journal={arXiv preprint arXiv:2207.05071},
  year={2022}
}

@article{chu2023qwen,
  title={Qwen-audio: Advancing universal audio understanding via unified large-scale audio-language models},
  author={Chu, Yunfei and Xu, Jin and Zhou, Xiaohuan and Yang, Qian and Zhang, Shiliang and Yan, Zhijie and Zhou, Chang and Zhou, Jingren},
  journal={arXiv preprint arXiv:2311.07919},
  year={2023}
}

@article{hsu2021hubert,
  title={Hubert: Self-supervised speech representation learning by masked prediction of hidden units},
  author={Hsu, Wei-Ning and Bolte, Benjamin and Tsai, Yao-Hung Hubert and Lakhotia, Kushal and Salakhutdinov, Ruslan and Mohamed, Abdelrahman},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={29},
  pages={3451--3460},
  year={2021},
  publisher={IEEE}
}
@article{zhang2023google,
  title={Google usm: Scaling automatic speech recognition beyond 100 languages},
  author={Zhang, Yu and Han, Wei and Qin, James and Wang, Yongqiang and Bapna, Ankur and Chen, Zhehuai and Chen, Nanxin and Li, Bo and Axelrod, Vera and Wang, Gary and others},
  journal={arXiv preprint arXiv:2303.01037},
  year={2023}
}
@inproceedings{radford2023robust,
  title={Robust speech recognition via large-scale weak supervision},
  author={Radford, Alec and Kim, Jong Wook and Xu, Tao and Brockman, Greg and McLeavey, Christine and Sutskever, Ilya},
  booktitle={International Conference on Machine Learning},
  pages={28492--28518},
  year={2023},
  organization={PMLR}
}
@inproceedings{aljundi2018memory,
  title={Memory aware synapses: Learning what (not) to forget},
  author={Aljundi, Rahaf and Babiloni, Francesca and Elhoseiny, Mohamed and Rohrbach, Marcus and Tuytelaars, Tinne},
  booktitle={Proceedings of the European conference on computer vision (ECCV)},
  pages={139--154},
  year={2018}
}
@article{kirkpatrick2017overcoming,
  title={Overcoming catastrophic forgetting in neural networks},
  author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
  journal={Proceedings of the national academy of sciences},
  volume={114},
  number={13},
  pages={3521--3526},
  year={2017},
  publisher={National Acad Sciences}
}


@inproceedings{bu2017aishell,
  title={Aishell-1: An open-source mandarin speech corpus and a speech recognition baseline},
  author={Bu, Hui and Du, Jiayu and Na, Xingyu and Wu, Bengu and Zheng, Hao},
  booktitle={2017 20th conference of the oriental chapter of the international coordinating committee on speech databases and speech I/O systems and assessment (O-COCOSDA)},
  pages={1--5},
  year={2017},
  organization={IEEE}
}

@article{zhao2020open,
  title={An open speech resource for Tibetan multi-dialect and multitask recognition},
  author={Zhao, Yue and Xu, Xiaona and Yue, Jianjian and Song, Wei and Li, Xiali and Wu, Licheng and Ji, Qiang},
  journal={International Journal of Computational Science and Engineering},
  volume={22},
  number={2-3},
  pages={297--304},
  year={2020},
  publisher={Inderscience Publishers (IEL)}
}
@article{liu2023sparsely,
  title={Sparsely Shared LoRA on Whisper for Child Speech Recognition},
  author={Liu, Wei and Qin, Ying and Peng, Zhiyuan and Lee, Tan},
  journal={arXiv preprint arXiv:2309.11756},
  year={2023}
}
@inproceedings{THUGY20_2015,
  title={THUGY20: A free Uyghur speech database},
  author={Askar Roze, Shi Yin, Zhiyong Zhang, Dong Wang, Askar Hamdulla},
  booktitle={NCMMSC'15},
  year={2015}
}
@inproceedings{XBMU-AMDO31,
  title={{XBMU-AMDO31:An open source of Amdo Tibetan speech
database and speech recognition baseline system}},
  author={Senyan Li, Guanyu Li, Jiewen Ning},
  booktitle={National Conference on Man-Machine Speech Communication,NCMMSC2022},
  year={2022},
}
@inproceedings{zhang2022wenetspeech,
  title={Wenetspeech: A 10000+ hours multi-domain mandarin corpus for speech recognition},
  author={Zhang, Binbin and Lv, Hang and Guo, Pengcheng and Shao, Qijie and Yang, Chao and Xie, Lei and Xu, Xin and Bu, Hui and Chen, Xiaoyu and Zeng, Chenchen and others},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6182--6186},
  year={2022},
  organization={IEEE}
}
@article{ardila2019common,
  title={Common voice: A massively-multilingual speech corpus},
  author={Ardila, Rosana and Branson, Megan and Davis, Kelly and Henretty, Michael and Kohler, Michael and Meyer, Josh and Morais, Reuben and Saunders, Lindsay and Tyers, Francis M and Weber, Gregor},
  journal={arXiv preprint arXiv:1912.06670},
  year={2019}
}
@inproceedings{zenke2017continual,
  title={Continual learning through synaptic intelligence},
  author={Zenke, Friedemann and Poole, Ben and Ganguli, Surya},
  booktitle={International conference on machine learning},
  pages={3987--3995},
  year={2017},
  organization={PMLR}
}
@inproceedings{wang2023rehearsal,
  title={Rehearsal-free continual language learning via efficient parameter isolation},
  author={Wang, Zhicheng and Liu, Yufang and Ji, Tao and Wang, Xiaoling and Wu, Yuanbin and Jiang, Congcong and Chao, Ye and Han, Zhencong and Wang, Ling and Shao, Xu and others},
  booktitle={Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={10933--10946},
  year={2023}
}
@inproceedings{hermjakob-etal-2018-box,
    title = "Out-of-the-box Universal {R}omanization Tool uroman",
    author = "Hermjakob, Ulf  and
      May, Jonathan  and
      Knight, Kevin",
    editor = "Liu, Fei  and
      Solorio, Thamar",
    booktitle = "Proceedings of {ACL} 2018, System Demonstrations",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P18-4003",
    doi = "10.18653/v1/P18-4003",
    pages = "13--18",
    abstract = "We present uroman, a tool for converting text in myriads of languages and scripts such as Chinese, Arabic and Cyrillic into a common Latin-script representation. The tool relies on Unicode data and other tables, and handles nearly all character sets, including some that are quite obscure such as Tibetan and Tifinagh. uroman converts digital numbers in various scripts to Western Arabic numerals. Romanization enables the application of string-similarity metrics to texts from different scripts without the need and complexity of an intermediate phonetic representation. The tool is freely and publicly available as a Perl script suitable for inclusion in data processing pipelines and as an interactive demo web page.",
}

@article{razdaibiedina2023progressive,
  title={Progressive prompts: Continual learning for language models},
  author={Razdaibiedina, Anastasia and Mao, Yuning and Hou, Rui and Khabsa, Madian and Lewis, Mike and Almahairi, Amjad},
  journal={arXiv preprint arXiv:2301.12314},
  year={2023}
}
@article{chaudhry2019tiny,
  title={On tiny episodic memories in continual learning},
  author={Chaudhry, Arslan and Rohrbach, Marcus and Elhoseiny, Mohamed and Ajanthan, Thalaiyasingam and Dokania, Puneet K and Torr, Philip HS and Ranzato, Marc'Aurelio},
  journal={arXiv preprint arXiv:1902.10486},
  year={2019}
}
@inproceedings{aljundi2018memory,
  title={Memory aware synapses: Learning what (not) to forget},
  author={Aljundi, Rahaf and Babiloni, Francesca and Elhoseiny, Mohamed and Rohrbach, Marcus and Tuytelaars, Tinne},
  booktitle={Proceedings of the European conference on computer vision (ECCV)},
  pages={139--154},
  year={2018}
}
@article{winata2023overcoming,
  title={Overcoming catastrophic forgetting in massively multilingual continual learning},
  author={Winata, Genta Indra and Xie, Lingjue and Radhakrishnan, Karthik and Wu, Shijie and Jin, Xisen and Cheng, Pengxiang and Kulkarni, Mayank and Preotiuc-Pietro, Daniel},
  journal={arXiv preprint arXiv:2305.16252},
  year={2023}
}
@article{kirkpatrick2017overcoming,
  title={Overcoming catastrophic forgetting in neural networks},
  author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
  journal={Proceedings of the national academy of sciences},
  volume={114},
  number={13},
  pages={3521--3526},
  year={2017},
  publisher={National Acad Sciences}
}
@article{chaudhry2019tiny,
  title={On tiny episodic memories in continual learning},
  author={Chaudhry, Arslan and Rohrbach, Marcus and Elhoseiny, Mohamed and Ajanthan, Thalaiyasingam and Dokania, Puneet K and Torr, Philip HS and Ranzato, Marc'Aurelio},
  journal={arXiv preprint arXiv:1902.10486},
  year={2019}
}
@article{mai2020batch,
  title={Batch-level experience replay with review for continual learning},
  author={Mai, Zheda and Kim, Hyunwoo and Jeong, Jihwan and Sanner, Scott},
  journal={arXiv preprint arXiv:2007.05683},
  year={2020}
}
@article{rolnick2019experience,
  title={Experience replay for continual learning},
  author={Rolnick, David and Ahuja, Arun and Schwarz, Jonathan and Lillicrap, Timothy and Wayne, Gregory},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  year={2019}
}

@inproceedings{vander2022continual,
  title={Continual learning for monolingual end-to-end automatic speech recognition},
  author={Vander Eeckt, Steven and Van Hamme, Hugo},
  booktitle={2022 30th European Signal Processing Conference (EUSIPCO)},
  pages={459--463},
  year={2022},
  organization={IEEE}
}
@article{chang2021towards,
  title={Towards lifelong learning of end-to-end ASR},
  author={Chang, Heng-Jui and Lee, Hung-yi and Lee, Lin-shan},
  journal={arXiv preprint arXiv:2104.01616},
  year={2021}
}
@inproceedings{chang2021towards,
  author       = {Heng{-}Jui Chang and
                  Hung{-}yi Lee and
                  Lin{-}Shan Lee},
  editor       = {Hynek Hermansky and
                  Honza Cernock{\'{y}} and
                  Luk{\'{a}}s Burget and
                  Lori Lamel and
                  Odette Scharenborg and
                  Petr Motl{\'{\i}}cek},
  title        = {Towards Lifelong Learning of End-to-End {ASR}},
  booktitle    = {Interspeech 2021, 22nd Annual Conference of the International Speech
                  Communication Association, Brno, Czechia, 30 August - 3 September
                  2021},
  pages        = {2551--2555},
  publisher    = {{ISCA}},
  year         = {2021},
  url          = {https://doi.org/10.21437/Interspeech.2021-563},
  doi          = {10.21437/INTERSPEECH.2021-563},
  timestamp    = {Sat, 30 Sep 2023 09:49:02 +0200},
  biburl       = {https://dblp.org/rec/conf/interspeech/ChangLL21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}
@article{zhang2023adaptive,
  title={Adaptive budget allocation for parameter-efficient fine-tuning},
  author={Zhang, Qingru and Chen, Minshuo and Bukharin, Alexander and He, Pengcheng and Cheng, Yu and Chen, Weizhu and Zhao, Tuo},
  journal={arXiv preprint arXiv:2303.10512},
  year={2023}
}
@inproceedings{farajtabar2020orthogonal,
  title={Orthogonal gradient descent for continual learning},
  author={Farajtabar, Mehrdad and Azizan, Navid and Mott, Alex and Li, Ang},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={3762--3773},
  year={2020},
  organization={PMLR}
}
@article{wang2023orthogonal,
  title={Orthogonal subspace learning for language model continual learning},
  author={Wang, Xiao and Chen, Tianze and Ge, Qiming and Xia, Han and Bao, Rong and Zheng, Rui and Zhang, Qi and Gui, Tao and Huang, Xuanjing},
  journal={arXiv preprint arXiv:2310.14152},
  year={2023}
}




